Rehearsing Answers to Probable Questions with Perspective-Taking

Question answering (QA) has been a long-standing focus in the NLP field, predominantly addressing reading comprehension and common sense QA. However, scenarios involving the preparation of answers to probable questions during professional oral presentations remain underexplored. In this paper, we pioneer the examination of this crucial yet overlooked topic by utilizing real-world QA conversation transcripts between company managers and professional analysts. We explore the proposed task using three causal knowledge graphs (KGs) and three large language models (LLMs). This work provides foundational insights into the application of LLMs in professional QA scenarios, highlighting the importance of causal KGs and perspective-taking in generating effective responses.

==> sections/1_introduction.tex <==
\section{Introduction} % done 
Preparing in-person Q\&A responses is a routine task in various professional fields.
For instance, in corporate settings, responses often adopt an official tone, which may not fully meet the listener's expectations.
In the financial sector, earnings conference calls serve as a direct communication channel between company executives and financial analysts, providing essential insights into corporate strategies and performance. 
% These calls are vital for the flow of information in equity markets.
% They also offer critical platforms for company managers to engage with professional analysts. 
However, it is common for managers to prepare evasive responses to anticipated questions before these calls to protect the company's interests. Table~\ref{table:raw_example} showcases an example of original response from these calls, illustrating a situation where managers did not directly answer the questions, which highlights the significance of our improvements in guaranteeing transparent responses.
This paper introduces the Knowledge Graph Question Answering (KGQA) system, a novel approach designed to provide straightforward and precise answers.

\begin{table}[hbt!]
    \centering
    \small
    \begin{tabular}{@{}p{7.5cm}@{}}
    \toprule
    \textbf{Question} \\
    Do you think the timeframe for getting Forever 21 EBITDA positive will be similar to that of Aero? \\
    % \addlinespace
    \midrule
    % \addlinespace
    \textbf{Answer} \\
    I would say that -- it's a good question. And I would say it's a little more complicated in a little bigger business. And it depends on whether one or two of my guys are going to spend all this time in Los Angeles. So, I'm negotiating it right now, Linda. Stay tuned.  \\
    \bottomrule
    \end{tabular}
    \caption{Example of Original Question and Answer}
    \label{table:raw_example}
\end{table}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/LLM_eval.pdf}
    \caption{The framework of our LLMs evaluation.}
    \label{fig:eval_framework}
\end{figure}

In this work, we introduce a variety of innovative methods aimed at improving response generation.
We utilize Knowledge Graphs (KG) and the textual content from the presentation sections of earnings calls to generate direct, clear, and comprehensive responds for analysts' questions, rather than sidestepping them due to corporate strategic considerations.

Initially, we measured the similarity between the original responses provided by the managers and the generated responses with common evaluation methods, where the original responses are considered as ground truth.
The enhanced instruction-following capabilities of LLMs have recently positioned them as strong one for automated evaluation tasks \citep{chiang2023large, liu2023gpteval, huang2023chatgpt}. 
Given these capabilities, we also tackle the challenge of evaluating complex Question-Answering scenarios during earnings conference calls, as shown in \autoref{fig:eval_framework}. 
By simply instructing the LLMs on how to rate and giving the LLMs, the LLM can follow the instructions and provide a rating of the sample. Our methodology introduces a way to evaluate whether the question can be effectively addressed by the answer generated from LLMs.
The objective is to create a robust and precise evaluation framework. We evaluate the \textit{concreteness}, \textit{information richness}, \textit{relevance and accuracy} of the response. 
The dataset details are in Appendix~\ref{sec: LLM_eval_prompt}.

\input{tables/FR_elements}

Overall, our key contributions are outlined as follows:
\begin{enumerate}
    \item We construct the KG by exploiting data extracted from financial reports, creating a structured repository of financial information. 
    
    \item We develop the augmented LLM framework, which integrates external knowledge via the KG into our QA systems. This enhancement broadens the dimensions of responses. 

    \item Beyond basic automatic metrics, we employ LLM-eval to assess multiple dimensions of conversation quality. Moreover, we conduct evaluations with human judges by experts to further validate our findings.
\end{enumerate}
% All resources are available at GitHub. 




==> sections/2_related_work.tex <==
\section{Related Work}
In recent research, there has been a surge of interest in representing KGs as natural language passages. 
% \citet{wang2021gnn} emphasize the role of Graph Neural Networks (GNNs) in Question Answering (QA) systems. 
% -> retrieve subgraphs as additional input besides question. 
% -> However, this constrains retrieved knowledge in local subgraphs and discards more diverse triplets buried in KGs that are disconnected but useful for question answering. 
% \citet{li2023graph} propose a method to retrieve and prioritize relevant triplets from KGs, demonstrating improved QA performance. 
% \citet{ma2021open} introduce a framework for Open-Domain Question Answering (ODQA) that leverages both text and structured knowledge from sources like Wikipedia and Wikidata, showcasing substantial enhancements over baseline methods. 
% \citet{christmann2022conversational} present CONVINSE, a pipeline for Conversational Question Answering (ConvQA) over heterogeneous sources, integrating KGs, text corpora, and tables to enhance answer coverage and confidence. Their ConvMix benchmark and experiments underline the effectiveness of this approach.


% \cite{wang2021gnn} Question Answering (QA) has been a long-standing research topic in AI and NLP fields, and a wealth of studies have been conducted to attempt to equip QA systems with human-level reasoning capability. To approximate the complicated human reasoning process, state-of-the-art QA systems commonly use pre-trained language models (LMs) to access knowledge encoded in LMs together with elaborately designed modules based on Graph Neural Networks (GNNs) to perform reasoning over knowledge graphs (KGs). However, many problems remain open regarding the reasoning functionality of these GNN-based modules. Can these GNN-based modules really perform a complex reasoning process? Are they under- or over-complicated for QA? To open the black box of GNN and investigate these problems, we dissect state-of-the-art GNN modules for QA and analyze their reasoning capability. We discover that even a very simple graph neural counter can outperform all the existing GNN modules on CommonsenseQA and OpenBookQA, two popular QA benchmark datasets which heavily rely on knowledge-aware reasoning. Our work reveals that existing knowledge-aware GNN modules may only carry out some simple reasoning such as counting. It remains a challenging open problem to build comprehensive reasoning modules for knowledge-powered QA.

% \cite{li2023graph}: Answering complex questions often requires reasoning over knowledge graphs (KGs). State-of-the-art methods often utilize entities in questions to retrieve local subgraphs, which are then fed into KG encoder, e.g. graph neural networks (GNNs), to model their local structures and integrated into language models for question answering. However, this paradigm constrains retrieved knowledge in local subgraphs and discards more diverse triplets buried in KGs that are disconnected but useful for question answering. In this paper, we propose a simple yet effective method to first retrieve the most relevant triplets from KGs and then rerank them, which are then concatenated with questions to be fed into language models. Extensive results on both CommonsenseQA and OpenbookQA datasets show that our method can outperform state-of-the-art up to 4.6% absolute accuracy.

% \cite{ma2021open}: The retriever-reader framework is popular for open-domain question answering (ODQA) due to its ability to use explicit knowledge. Although prior work has sought to increase the knowledge coverage by incorporating structured knowledge beyond text, accessing heterogeneous knowledge sources through a unified interface remains an open question. While data-to-text generation has the potential to serve as a universal interface for data and text, its feasibility for downstream tasks remains largely unknown. In this work, we bridge this gap and use the data-to-text method as a means for encoding structured knowledge for ODQA. Specifically, we propose a verbalizer-retriever-reader framework for ODQA over data and text where verbalized tables from Wikipedia and graphs from Wikidata are used as augmented knowledge sources. We show that our Unified Data and Text QA, UDT-QA, can effectively benefit from the expanded knowledge index, leading to large gains over text-only baselines. Notably, our approach sets the single-model state-of-the-art on Natural Questions. Furthermore, our analyses indicate that verbalized knowledge is preferred for answer reasoning for both adapted and hot-swap settings.


% \cite{christmann2022conversational}: Conversational question answering (ConvQA) tackles sequential information needs where contexts in follow-up questions are left implicit. Current ConvQA systems operate over homogeneous sources of information: either a knowledge base (KB), or a text corpus, or a collection of tables. This paper addresses the novel issue of jointly tapping into all of these together, this way boosting answer coverage and confidence. We present CONVINSE, an end-to-end pipeline for ConvQA over heterogeneous sources, operating in three stages: i) learning an explicit structured representation of an incoming question and its conversational context, ii) harnessing this frame-like representation to uniformly capture relevant evidences from KB, text, and tables, and iii) running a fusion-in-decoder model to generate the answer. We construct and release the first benchmark, ConvMix, for ConvQA over heterogeneous sources, comprising 3000 real-user conversations with 16000 questions, along with entity annotations, completed question utterances, and question paraphrases. Experiments demonstrate the viability and advantages of our method, compared to state-of-the-art baselines.


% Produce corresponding answers to questions is a challenging task for both humans and machines. 

% Previous studies have primarily focused on ... , often centered around generating answer for ...

% \citet{ren2023towards}

% % 我哪裡不同
% In contrast to previous studies focusing on generating answer for ..., 
% our work proposes generating answer in live presentations. 
% % 不同之處
% There are distinct differences between these tasks. 
% % 現在也用 kg 生成 answer 的例子
% Although earnings conference calls have been widely studied for various tasks such ..., the answer generation task has received little attention. 
% Thus, our paper aims to fill this research gap by providing ... .

==> sections/4_prposed_pipeline.tex <==
\section{Methodology}
A crucial observation in our study is the significant role financial terminology plays in creating responses for a specific question. Our methodology emphasizes integrating these terms with additional, relevant information to ensure the authenticity of the answers provided. We aim to enhance the quality of responses by utilizing KG and incorporating data from presentations prepared prior to Q\&A sessions, 
aiming to deliver more effective and contextually relevant answers.

Recently, question-answering over KG has emerged as a research focus. 
% However, traditional KGs frequently fail to address the complexity of questions typical in earnings conference calls, which often involve detailed causal relationships among various financial events and phenomena.
However, traditional KGs frequently fail to address the complex details of casual relationships involving various financial events and phenomena, which are typical in earnings conference calls.
To overcome this challenge, we propose the development of a specialized causality graph tailored for this unique context, designed to support causal inference.
This specialized graph significantly improves the analysis in financial reports that demand a thorough exploration of cause and effect. 

This innovative approach distinguishes our methodology from traditional answer generation tasks that do not leverage causal reasoning. By focusing on causal connections, our strategy aims to deliver responses that are not only precise but also richly informed by the context of the query.

\subsection{Problem Setup}
We focus on LFQA tasks that require sophisticated model reasoning capabilities. For each instance in earnings conference calls dataset, we are provided with a question \( Q \) and a pre-call presentation \( P \). 
Additionally, we assume access to a knowledge graph \( G \), which offers potentially relevant information to formulate answers to each question. 
Given an example \( (Q, P) \) and a knowledge graph \( G \), our goal is to generate more accurate answers.

\subsection{Constructed Causal KG}
We focus on argument-unit identification in financial texts, a foundational step in enhancing text analysis and establishing a causal financial knowledge graph.
We developed a model to classify sentences into three categories that are critical for structuring logical arguments:
\begin{compactitem}
    \vspace{0.5em}
    \item Claim: A statement or assertion from a certain viewpoint that requires reasoning or proof.
    \item Premise: Provides reasons or evidence that support the claim.
    \item Scenario: Describes a hypothetical or actual situation to illustrate potential outcomes of decisions.
    \vspace{0.5em}
\end{compactitem}

Examples of each category, derived from manually annotated data, are detailed in Table~\ref{tab:financial-analysis}. 

Initially, we extracted sentences categorized as \textbf{Claim, Premise, and Scenario} from a substantial corpus of textual data.  

Utilizing a dataset comprising 21,904 training items and 7,595 test items, each manually annotated.
We fine-tuned a \textbf{RoBERTa-base} \cite{liu2019roberta} model to differentiate among these categories, achieving a test accuracy of approximately 90.78\%. 
The distribution of data is presented in Table~\ref{tab:data_distribution}. 
\input{tables/data_distribution}

Following this, we extracted financial terms from the sentences categorized as Premises (considered as causes) and also from the corresponding sentences categorized as Claims (considered as effects).  
This establishes direct causal relationships between financial terms.
These terms were then paired to form corresponding cause-and-effect pairs. 
These pairs were combined to construct a causal knowledge graph.


Additionally, we neutralized pairs exhibiting mutual causality—where "A causes B" and "B causes A"—to eliminate redundancy and contradictions, thereby refining the knowledge graph.
The refined Causal KG, purged of inconsistencies, now serves as a robust foundation for our question-answering tasks.

\subsection{Entity Retriever}
% \subsection{Entities from KG Retriever}
For knowledge graph, there are two main methods for integration with LLM. 
The first method involves selecting the top-n most relevant entities from the knowledge graph that represent effects deduced from the question as a cause. 
The second method involves incorporating all relevant entities from the knowledge graph into the LLM. We adopted the second method here since it preserve the most information.
% These integration strategies enhance the LLM’s ability to utilize the structured data from our knowledge graphs, thus improving its response capabilities in financial question-answering scenarios.

% In our approach, 
% the question acts as the causal trigger to deduce effect-related terms from the knowledge graph \( G \).
% We identify terms in \( G \) that are contextually relevant to the cause represented by the question \( Q \) and extract these terms. 
% These extracted entities are subsequently transformed into a passage corpus \( D \), ready for further processing and answer generation.
In our approach, we identify the terms that can be marked as cause entities from the questions, and retrieve the corresponding effect entities from the knowledge graph \(G\). 
These extracted entities are subsequently transformed into a passage corpus \( D \), ready for further processing and answer generation.
% 給圖

\subsection{Answer Generator}
LLMs possess the capability to perform zero-shot, closed-book question answering. 
However, this internalized knowledge may not always be accurate or comprehensive, occasionally leading to factually incorrect responses.
To mitigate this issue, we enhances the LLM's capabilities by integrating relevant facts from \( G \), specifically tailored to the input question. 
These facts are pre-appended to the original question to form a new, enriched prompt, which is then fed into the LLM for answer generation.
Our framework operates entirely in a zero-shot manner, eliminating the need for additional model training and aiming to bridge the gap between the LLM’s pre-stored knowledge and the factual accuracy required for domain-specific answer generation.

During the answer generation process, the LLM utilizes structured data from our knowledge graphs and information from presentations before Q\&A sections.
By incorporating these diverse data sources, the LLM is better equipped to deliver comprehensive and contextually relevant answers, thereby enhancing its effectiveness in financial question-answering scenarios.
We explore different input configurations to apply the LLM’s zero-shot capabilities, allowing the model to generate responses based solely on the provided input, without prior training on similar tasks. 



==> sections/5_experiment.tex <==
\section{Experiment}
\subsection{Experimental setups}
\paragraph{Dataset}
We evaluate our method on earnings conference calls datasets that require sophisticated model reasoning capabilities. 
Our dataset comprises 205 transcriptions of earnings conference calls sourced from Reuters
% \footnote{\href{https://ir.thomsonreuters.com/financial-information/quarterly-reports} {https://ir.thomsonreuters.com/financial-information/quarterly-reports}}
, featuring presentations from 179 different companies.
Our methodology generates answers based on the provided questions, presentations, and causal knowledge graph, with each question associated with the corresponding presentations from the Q\&A sessions of the earnings conference calls.

\paragraph{Financial Terms}
Our financial terms were sourced from two authoritative financial dictionaries: Investopedia Financial Terms Dictionary \footnote{\href{https://www.investopedia.com/financial-term-dictionary-4769738}{https://www.investopedia.com/financial-term-dictionary-4769738}} and Financial Times Lexicon \footnote{\href{https://markets.ft.com/glossary/searchLetter.asp?letter=C}{https://markets.ft.com/glossary/searchLetter.asp?letter=C}}. These comprehensive resources provided a total of 4,824 unique financial terms.


\paragraph{Knowledge Graph}
We have developed a unique knowledge graph, referred to as \textbf{KG}, from Financial Terms, we established 41,007 pairs of cause-and-effect relationships. These pairs form the backbone of our causal knowledge graph, enabling detailed analysis and understanding of financial dynamics.

In addition, we incorporate three other knowledge graphs from the framework introduced by \citet{xu2024framework}. Our objective is to conduct a comparative analysis of these knowledge graphs, as detailed in Table~\ref{tab:KGs}. 
Her comprehensive framework significantly enhances our ability to efficiently analyze and respond to complex queries, thus facilitating more informed decision-making in financial contexts.

\begin{compactitem}
    \vspace{0.5em}
    \item \textbf{FinCaKG}: FinCaKG-FR, FinCaKG-ECT, and FinCaKG-AR are frameworks introduced by \citet{xu2024framework}. The FinCaKG-FR is constructed using financial reports as the primary corpus, facilitating the development of the Financial Causal Knowledge Graph (FinCaKG). As for FinCaKG-ECT and FinCaKG-AR, they are KG extended from FinCaKG-FR by applying earnings call transcripts and analyst reports as additional corpora.
    \item \textbf{KG}: Our KG. 
    \vspace{0.5em}
\end{compactitem}

\input{tables/KGs}

\paragraph{Language Models}

% "Models" for prompting 
% 1. T5 - 0.8B/ 3B/ 11B (not yet)
% 2. T0 - 3B/ 11B (not yet)
% 3. GPT-3 - 6.7B/ 175B
% 4. OPT - 2.7B/ 6/7B/ 13B

% 1. No knowledge: naive LM prompting 
% 2. With Knowledge: add all 
% 3. Random Knowledge: randomly sample K (not yet)
% 4. Popular Knowledge: augments the K popular (not yet)
% 5. Generated Knowledge: extract from LLM themselves (not yet)
% In our experiments, we employ a prompt-based approach to enable  LLMs to generate financial answers.
% We systematically vary the content of the prompts to include different combinations of data, such as specific details from earnings conference call presentations and elements from the causal knowledge graph. 
% This methodology allows us to assess how various types of information affect the quality of the responses generated by the models.
% Specifically, we explore the effectiveness of different data integrations by testing prompts with varied levels of information to identify the most effective configurations. 
The LLMs used in our study include GPT-3.5, Gemini 1.0 Pro via their respective APIs, and the open-source model LLaMA 3. 
Our objective is to determine which data types most enhance the LLMs' ability to produce optimal outcomes in financial contexts.

We investigate four distinct configurations for data integration in the prompts used with LLMs:
These configurations are: (1) No presentation and no knowledge graph, (2) Presentation without knowledge graph, (3) Knowledge graph without presentation, and (4) Both presentation and knowledge graph included. 
This structured approach enables us to systematically analyze how different combinations of information impact the models’ ability to deliver accurate and insightful responses.

% In this subsection, we explain three zero-shot LM
% prompting baselines and our framework.
% 2. prompt 下的方式
% \paragraph{Naive Prompting} This is a baseline where the language model generates answers from input questions without any additional knowledge augmentation from KGs.

% \paragraph{Full Knowledge Augmentation} This is a baseline where the language model's prompts are augmented with all relevant related entities connected to the entities mentioned in the question.

% \paragraph{Selective Knowledge Augmentation} This is a baseline where the language model's prompts are augmented with a limited number of related terms connected to the entities mentioned in the question.

% evaluation
\input{tables/main_results}

\subsection{Automatic Evaluation Metric}
To evaluate the generated answers in response to specific questions and their alignment with ground truth answers, we utilize a set of metrics classified into two main categories.
First, the N-gram Based Metrics assess the literal text overlap between the generated and reference answers, focusing on surface-level textual similarities. 
Second, the Contextual Semantics Metrics evaluate the semantic consistency and contextual relevance between the generated answers and the ground truth. This approach provides a deeper understanding of answer quality, going beyond simple word matching to ensure a thorough evaluation of the content's relevance and accuracy. 
...

\subsubsection{N-gram Based Metrics}
% This category includes metrics that analyze the textual overlap and precision of n-grams between the generated text and the ground truth, focusing on literal accuracy and structural similarity.
We use metrics like \textbf{ROUGE} \cite{lin2004rouge}  and \textbf{BLEU} \cite{zhang2019bertscore} evaluate the extent of n-gram overlap and precision, respectively, focusing on how comprehensively and accurately the generated content captures essential information from the references.

\subsubsection{Contextual Semantics Metrics}
Beyond traditional metrics like BLEU and ROUGE, we employ advanced metrics to capture the nuances of language and the depth of understanding in generated answers. These metrics include \textbf{METEOR} \cite{banerjee2005meteor}, which assesses semantic similarity; \textbf{QuestEval} \cite{scialom2021questeval}, which evaluates faithfulness to the source content; and \textbf{BERTscore} \cite{zhang2019bertscore}, a pre-trained model-based metric that measures the contextual alignment of the generated text with the ground truth. 
Together, these tools provide a comprehensive analysis, revealing how closely the generated text matches the intended meaning and contextual accuracy required by the original queries.
% bigger one 
% \begin{figure*}[hbt!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/LLM_eval.pdf}
%     \caption{The framework of our LLMs evaluation.}
%     \label{fig:eval_framework}
% \end{figure*}

\subsection{Advanced Evaluation Metric}
 While automatic evaluation metrics offer initial insights into the quality of generated answers compared to reference answers, 
 they often fail to capture the full complexity and nuance.
 To address these shortcomings, this section introduces Term Ratio Metrics, LLM Evaluation using GPT-4~\citep{openai2023gpt4}, and Human Evaluation. 
 These metrics are designed to provide a more comprehensive analysis of the text, enabling a deeper understanding of contextual relevance of the generated content.

\subsubsection{Term Ratio Metrics}
This metric evaluates the relevance and richness of terms in generated answers (\(GA\)) relative to the reference answer (\(RA\)), that is, the ground truth, by examining three key aspects:

\begin{enumerate}
    \item The proportion of unique terms in \(GA\) compared to \(RA\), providing an overall comparison.
    \item The occurrence of question terms in the answers, examining basic relevancy.
    \item The presence of inferential terms not mentioned in the questions, indicating deeper insights.
\end{enumerate}

Each \(GA\) includes a list of financial terms \(GA_{\text{Terms}}\), 
and similarly, each \(RA\) also contains a list of financial terms \(RA_{\text{terms}}\). 
The list of financial terms appearing in the question (\(Q\)) is denoted as \(Q_{\text{terms}}\). 
We analyze the relationships between these term sets by examining their intersections and differences, providing insight into both the straightforward relevance and inferential depth of the responses.

The \textbf{Content Diversity Ratio (CDR)} quantifies the uniqueness of terms in the generated answers compared to the ground truth:
\begin{equation}
\small\text{CDR} = \frac{\left|GA_{\text{terms}}\right|}{{\left|RA_{\text{terms}}\right|}} 
\end{equation}
\vspace{0.3cm}

The \textbf{Question-Answer Alignment Ratio (QAR)} measures the overlap of terms between the question and the answers, assessing direct relevance:
\begin{equation}
\small\text{QAR} = \frac{\left|GA_{\text{terms}} \cap Q_{\text{terms}}\right|}{\left|RA_{\text{terms}} \cap Q_{\text{terms}}\right|} 
\end{equation}
\vspace{0.3cm}

The \textbf{Inferential Insight Ratio (IIR)} is determined by the proportion of unique terms in the answers that do not appear in the question, offering insights into the depth of the generated content:
\begin{equation}
\small\text{IIR} =  \frac{\left|GA_{\text{terms}} \setminus Q_{\text{terms}}\right|}{\left|RA_{\text{terms}} \setminus Q_{\text{terms}}\right|} 
\end{equation}
\vspace{0.3cm}

\subsubsection{LLM as an Evaluation Metric} 
We propose using LLMs as an automatic evaluation metric, where LLMs are tasked with rating samples based on specific attributes: Concreteness, Information Richness, and Relevance and Accuracy. 

\textbf{Concreteness} evaluates the level of detail in an answer. High scores are reserved for responses that provide detailed numerical data and empirical evidence, medium scores for those with some specifics, and low scores for vague answers lacking detailed examples.
\textbf{Information Richness} measures the extent and breath of information in a response. Responses that offer a comprehensive background, extensive analysis, and cover a wide range of ideas are rated highly. Medium scores go to responses with fair information but limited in some areas, and low scores are given to those with minimal and superficial information.
\textbf{Relevance and Accuracy} assess how directly and accurately an answer addresses the posed question. The highest score is reserved for responses that directly and accurately address the entire question, demonstrating both high relevance and accuracy. A medium score is applied to answers that somewhat address the question but may lack full relevance or contain some inaccuracies. The lowest score is given to responses that are irrelevant or inaccurate.

For our evaluations, we employ a comprehensive, multi-dimensional approach designed for our open-domain dialogues. We choose GPT-4 (OpenAI, 2022) for its robust capabilities. Drawing inspiration from \citet{chiang2023large}, our framework incorporates a single prompt that merges dialogue context with the generated responses. The evaluation process involves providing the LLM with descriptions of the rating task, definitions and rating criteria for the attributes to be rated, along with a sentence prompting the LLM to deliver the rating. This technique allows for efficient and precise measurement across multiple dimensions, with scores ranging from 0 to 10. By leveraging these criteria, LLMs can provide structured and consistent evaluations of text. 

% , as illustrated in \autoref{fig:eval_framework}. 
% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/LLM_eval.pdf}
%     \caption{The framework of our LLMs evaluation.}
%     \label{fig:eval_framework}
% \end{figure}

\subsubsection{Human Evaluation}
To ensure consistency in our evaluation process, we ask experts to apply the same set of metrics used in the LLM evaluation to human evaluations. This uniform approach allows for direct comparison between human and LLM results, enabling us to confirm the alignment and validity of outcomes across different evaluators.
\input{tables/different_kg_results}

==> sections/6_experiment_result.tex <==
\vspace{-0.05in}
\section{Experimental Results}
\label{sec:exp}
\vspace{-0.075in}
% automated metrics 
The experimental results, outlined in Table~\ref{tab:main_results}, are obtained by a range of automated evaluation metrics. 
These results emphasize the impact of integrating KG and presentation data on model performance.
It's important to note that these evaluations, which compare generated responses to those from managers during earnings calls, may not always align perfectly with analyst queries. 
Therefore, the scores should be regarded as indicative benchmarks, not definitive assessments of effectiveness.

Our analysis across different language models, consistently demonstrates that integrating presentation data significantly enhances answer quality. 
In contrast, solely using knowledge graphs sometimes leads to less accurate responses. 
This indicates that presentation data typically boosts the effectiveness of generated answers more than knowledge graphs. 
However, the lower performance associated with using only KGs might stem from insufficient content. 
Results consistently show that integrating presentation data substantially improves answer quality, while the use of knowledge graphs can sometimes yield less accurate responses. 
When presentation data and KGs are combined, the additional insights gained from the KG can effectively deepen the quality of the responses, indicating a synergistic effect that enhances overall answer.

In addition to our proposed KG, we also experimented with three other knowledge graphs under the FinCaKG framework. Below are the comparative results for comparison in Table~\ref{tab:different_kg_results}. ***

The LLM evaluations, presented in Table~\ref{tab:results_GPT4}, were conducted under budget considerations, so we only evaluated the outcomes generated by GPT-3.5 as a representative example.
We found that these results align with the methods used in automatic evaluations, indicating that answers incorporating presentation data typically outperform those that do not. However, including a knowledge graph often leads to misleading outcomes.
\input{tables/gpt4_results}

In our human annotation process, we noticed that managers frequently avoid addressing the question on point in their responses, as detailed in Table~\ref{tab:human}.
\input{tables/human_eval}
During the human annotation process, we analyzed the quality of responses under different data configurations. 
Insights revealed that responses were most straightforward and direct when neither KGs nor presentations were used.  % No KG, No presentation  
However, using only a knowledge graph increased the breadth of responses, covering more relevant content and details. % Have KG, No presentation  
In contrast, employing only a presentation enhanced the depth, leading to more detailed and specific answers. % No KG, Have presentation  
Notably, when both a knowledge graph and a presentation were used together, there was a significant improvement in both the breadth and depth of responses. % Have KG, Have presentation  
This was observed as the knowledge graph could expand on and delve deeper into points mentioned in the presentation, thereby enriching the overall quality of responses. 
These findings validate the effectiveness and applicability of our evaluation framework, highlighting how different data inputs can significantly affect the quality of answers.











==> sections/7_conclusion.tex <==
\section{Conclusion}
% This paper introduces the novel task of KGQA and explores its potential applications in generating answers based on a combination of questions, presentation transcripts, and knowledge graphs.  
% We identify several deficiencies in the QA process of earnings calls. 
% Our findings provide a valuable starting point for future research in KGQA.


==> tables/FR_elements.tex <==
\begin{table*}[hbt!]
    \centering
    \small
    \begin{tabular}{@{}lp{6cm}p{8cm}@{}} % Adjusted column width for better fit
    \toprule
         \textbf{} & \multicolumn{1}{c}{\textbf{Content}} & \multicolumn{1}{c}{\textbf{Description}} \tabularnewline 
    \midrule % Solid line after the header
        \textbf{Premise} & ``Largan’s share price is up 45\% since its May trough due to high expectations on iPhone 5.'' & This sentence describes the market expectations driving the stock price, setting the background for further analysis. \\
    \noalign{\vskip 0.5ex}\cdashline{1-3}\noalign{\vskip 0.75ex} % Dashed line after each entry
        \textbf{Scenario} & ``Weakening customer base could dampen Largan’s growth momentum in spite of strong smartphone industry growth.'' & This scenario outlines how, despite overall strong growth in the smartphone industry, a weakening customer base could impede the company's growth momentum. \\
    \noalign{\vskip 0.5ex}\cdashline{1-3}\noalign{\vskip 0.75ex}
        \textbf{Claim} & ``While we expect more positive news flow in the coming quarters, we would suggest investors sell into strength.'' & Based on the premise and scenario described, the recommendation is for investors to sell their shares while the stock price is strong. \\
    \bottomrule
    \end{tabular}
    \caption{Analysis of Financial Reporting Elements}
    \label{tab:financial-analysis}
\end{table*}

% --------------------------


==> tables/KGs.tex <==
\begin{table}[h]
\small
\centering
\resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{l|cccccc}
    \toprule
    \textbf{} & \textbf{KG} & \textbf{FinCaKG-FR} & \textbf{FinCaKG-ECT} & \textbf{FinCaKG-AR}\\
    \midrule
    \text{Entities} & 4,824 & 1,717 & 546 & 199 \\ 
    \text{Relations} & 41,007 & 11,633 & 1,802 & 283  \\  
    \bottomrule
    \end{tabular}
}
% \caption{Four KGs}
% The best scores are emphasized in bold, while underlined values indicate improvements over the original \textsc{answer}, showcasing the model's adaptability to different settings.}
\caption{Comparative Overview of Knowledge Graphs: This table presents a detailed comparison of the four knowledge graphs used in our study, including the KG and FinCaKG variants (FR, ECT, AR).}

\label{tab:KGs}
\end{table}


==> tables/case_study.tex <==
\setstcolor{red}

\begin{table*}[t!]\
\small
\centering
\caption{\small \textbf{Generation examples} of the prompted GPT-3.5 for the input question with augmented triples from the retriever, where, in the last row, we change the knowledge of augmented facts to see whether the model is able to adapt to the changed knowledge.}
\resizebox{1.00\textwidth}{!}{
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{lll}

\toprule
\multicolumn{3}{p{\textwidth}}{\textbf{Question}: Where did Alex Chilton die?} \\

\multicolumn{3}{p{\textwidth}}{\textbf{Retrieved triples}: (Alex Chilton, place of death, \hlyellow{New Orleans}), (Alex Chilton, manner of death, natural causes), (Alex Chilton, cause of death, \hlpink{myocardial infarction}), (Alex Chilton, date of death, time: \hlgreen{+2010-03-17}), ...} \\

\multicolumn{3}{p{\textwidth}}{\textbf{Answer}: \hlyellow{New Orleans}} \\

\midrule
{} & \multicolumn{1}{c}{\textbf{Prompts}} & \multicolumn{1}{c}{\textbf{Outputs}} \\
\midrule

\textbf{No Knowledge}
& \multicolumn{1}{p{0.54\textwidth}}{Question: Where did Alex Chilton die? Answer:}  
&  \multicolumn{1}{p{0.45\textwidth}}{Alex Chilton died in a \st{car accident} on \st{February 10, 1979}.} \\

\noalign{\vskip 0.5ex}\cdashline{0-2}\noalign{\vskip 0.75ex}

\multirow{6}{*}{\textbf{KAPING (Ours)}} 
& \multicolumn{1}{p{0.54\textwidth}}{Below are facts in the form of the triple meaningful to answer the question. ... (Alex Chilton, date of death, time: \hlgreen{+2010-03-17}) (Alex Chilton, cause of death, \hlpink{myocardial infarction}) (Alex Chilton, manner of death, natural causes) (Alex Chilton, place of death, \hlyellow{New Orleans})
Question: Where did Alex Chilton die? Answer:}  
&  \multicolumn{1}{p{0.45\textwidth}}{Alex Chilton died on \hlgreen{March 17, 2010} in \hlyellow{New Orleans}, Louisiana due to a \hlpink{myocardial infarction}.} \\

\noalign{\vskip 0.5ex}\cdashline{0-2}\noalign{\vskip 0.75ex}


\multirowcell{6}[-0.0ex][l]{\textbf{KAPING (Ours)} \\ \textbf{w/ Knowledge Change}} 
& \multicolumn{1}{p{0.54\textwidth}}{Below are facts in the form of the triple meaningful to answer the question. ... (Alex Chilton, date of death, time: \hlgreen{+2000-09-01}) (Alex Chilton, cause of death, \hlpink{pancreatic cancer}) (Alex Chilton, manner of death, natural causes) (Alex Chilton, place of death, \hlyellow{Los Angeles})
Question: Where did Alex Chilton die? Answer:}  
&  \multicolumn{1}{p{0.45\textwidth}}{Alex Chilton died in \hlyellow{Los Angeles}, California on \hlgreen{September 1, 2000} from \hlpink{pancreatic cancer}.} \\

\bottomrule
\end{tabular}
}

\label{tab:case_study}
\vspace{-0.125in}
\end{table*}


==> tables/data_distribution.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{@{}lrrrr@{}} 
    \toprule
    \textbf{Label} & \textbf{Train} & \textbf{Dev} & \textbf{Test} & \textbf{Whole} \\
    \midrule
    % Premise(0), Scenario(2), Claim(1)
    Premise   & 9,433          & 1,048        & 4,095         & 14,576 \\
    Scenario  & 5,537          & 616          & 2,039         & 8,192  \\
    Claim    & 4,743          & 527          & 1,461         & 6,731  \\
    \midrule
    \textbf{Total} & \textbf{19,713} & \textbf{2,191} & \textbf{7,595} & \textbf{29,499} \\
    \bottomrule
\end{tabular}
\caption{Data statistics of argument unit identification}
\label{tab:data_distribution}
\end{table}


==> tables/different_kg_results.tex <==
% \begin{table}[hbt!]
% \centering
% \resizebox{0.5\textwidth}{!}{%
%     \begin{tabular}{lccccc}
%     \toprule
%     \textbf{} &\textbf{ROUGE-1} &\textbf{ROUGE-2} & \textbf{ROUGE-L} \\
%     \midrule
%     {\textit{\textbf{FinCaKG-FR}}} & 22.69 & 3.57 & 12.31 \\
%     % \midrule
%     {\textit{\textbf{FinCaKG-ECT}}} & 25.50 & 4.23 & 13.64 \\
%     % \midrule
%     {\textit{\textbf{KFinCaKG-AR}}} & 24.88 & 3.95 & 13.27 \\
%     \midrule
%     {\textit{\textbf{KG}}} & 27.26 & 4.96 & 14.43 \\
%     \bottomrule
%     \end{tabular}
% }
% \caption{\textbf{Evaluation results of different KGs.}}

% \label{tab:results_KGs}

% \end{table}

\begin{table*}[t!]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccca}
% \begin{tabular}{l|cc|ccccccc|ccca}
\toprule

& \multicolumn{2}{c}{} & \multicolumn{4}{c}{\bf N-gram Based} & \multicolumn{3}{c}{\bf Contextual Semantics} & \multicolumn{3}{c}{\bf Term} \\
\cmidrule(l{2pt}r{2pt}){4-7} \cmidrule(l{2pt}r{2pt}){8-10}  \cmidrule(l{2pt}r{2pt}){11-13}

\textbf{} & \textbf{KG} & \textbf{PRE} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{BLEU} & \textbf{METEOR} & \textbf{QuestEval} & \textbf{BERTscore} & \textbf{CDR} & \textbf{QDR} & \textbf{IIR} & \textbf{Length} \\

\midrule
% \midrule
\multirow{2}{*}{\textit{\textbf{FinCaKG-ECT}}} 
& \cmark & \xmark & 26.45 & 4.19 & 13.82 \\
& \cmark & \cmark & 28.03 & 4.48 & 14.00 \\
% \noalign{\vskip 0.5ex}\cdashline{2-14}\noalign{\vskip 0.75ex} % dotted line
% & \cmark &  \xmark & \\
% & \cmark & \cmark & \\
\midrule


\multirow{2}{*}{\textit{\textbf{FinCaKG-FR}}} 
& \cmark &  \xmark & 26.63 & 4.21 & 13.89 \\
& \cmark & \cmark & 27.90 & 4.43 & 14.00 \\
% \noalign{\vskip 0.5ex}\cdashline{2-14}\noalign{\vskip 0.75ex} % dotted line
% & \cmark &  \xmark & \\
% & \cmark & \cmark & \\
\midrule


% \multirow{2}{*}{\textit{\textbf{FinCaKG-AR}}}
% & \cmark &  \xmark & \\
% & \cmark & \cmark & \\
% \noalign{\vskip 0.5ex}\cdashline{2-15}\noalign{\vskip 0.75ex} % dotted line
% & \cmark &  \xmark & \\
% & \cmark & \cmark & \\
% \midrule

\multirow{2}{*}{\textit{\textbf{KG}}}
& \cmark &  \xmark & 27.11 & 4.35 & 14.12 & 0.54 & 19.33 & 31.77 & 83.70 & 17.69 & 41.79 & 8.72 & 112 \\
& \cmark & \cmark & 27.85 & 4.28 & 13.86 & 0.73 & 16.66 & 30.18 & 82.97 & 24.06 & 38.69 & 18.54 & 185 \\
% \noalign{\vskip 0.5ex}\cdashline{2-14}\noalign{\vskip 0.75ex} % dotted line
% & \cmark &  \xmark & \\
% & \cmark & \cmark & \\

\bottomrule

\end{tabular}

}
\caption{\textbf{Evaluation results of different KGs. (GPT-3.5)}}
\label{tab:different_kg_results}
\end{table*}




\begin{table*}[t!]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccca}
% \begin{tabular}{l|cc|ccccccc|ccca}
\toprule

& \multicolumn{2}{c}{} & \multicolumn{4}{c}{\bf N-gram Based} & \multicolumn{3}{c}{\bf Contextual Semantics} & \multicolumn{3}{c}{\bf Term} \\
\cmidrule(l{2pt}r{2pt}){4-7} \cmidrule(l{2pt}r{2pt}){8-10}  \cmidrule(l{2pt}r{2pt}){11-13}

\textbf{} & \textbf{KG} & \textbf{PRE} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{BLEU} & \textbf{METEOR} & \textbf{QuestEval} & \textbf{BERTscore} & \textbf{CDR} & \textbf{QDR} & \textbf{IIR} & \textbf{Length} \\

\midrule
% \midrule
\multirow{2}{*}{\textit{\textbf{FinCaKG-ECT}}} 
& \cmark &  \xmark & 33.76 & 6.07 & 15.16 \\
& \cmark & \cmark & 27.93 & 3.96 & 12.98 \\
\midrule

\multirow{2}{*}{\textit{\textbf{FinCaKG-FR}}} 
& \cmark & \xmark & 33.68 & 6.13 & 15.40 \\
& \cmark & \cmark & 27.51 & 3.82 & 12.98 \\
\midrule

\multirow{2}{*}{\textit{\textbf{KG}}}
& \cmark &  \xmark & 28.95 & 4.72 & 13.55 & 0.82 & 14.69 & 28.55 & 82.27 & 16.53 & 24.21 & 13.65 & 313\\
& \cmark & \cmark & 28.28 & 4.18 & 13.30 & 0.54 & 13.77 & 29.57 & 81.81 & 19.08 & 18.62 & 17.31 & 303\\

\bottomrule

\end{tabular}

}
\caption{\textbf{(Llama)}}
\label{tab:different_kg_results}
\end{table*}




\begin{table*}[t!]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccca}
% \begin{tabular}{l|cc|ccccccc|ccca}
\toprule

& \multicolumn{2}{c}{} & \multicolumn{4}{c}{\bf N-gram Based} & \multicolumn{3}{c}{\bf Contextual Semantics} & \multicolumn{3}{c}{\bf Term} \\
\cmidrule(l{2pt}r{2pt}){4-7} \cmidrule(l{2pt}r{2pt}){8-10}  \cmidrule(l{2pt}r{2pt}){11-13}

\textbf{} & \textbf{KG} & \textbf{PRE} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{BLEU} & \textbf{METEOR} & \textbf{QuestEval} & \textbf{BERTscore} & \textbf{CDR} & \textbf{QDR} & \textbf{IIR} & \textbf{Length} \\

\midrule
% \midrule
\multirow{2}{*}{\textit{\textbf{FinCaKG-ECT}}} 
& \cmark & \xmark & \\
& \cmark & \cmark & \\

\midrule

\multirow{2}{*}{\textit{\textbf{FinCaKG-FR}}} 
& \cmark &  \xmark & \\
& \cmark & \cmark & \\

\midrule

\multirow{2}{*}{\textit{\textbf{KG}}}
& \cmark &  \xmark & 27.26 & 4.96 & 14.43 & 0.81 & 18.86 & 31.65 & 83.86 & 15.61 & 41.70 & 6.47 & 107\\
& \cmark & \cmark & 24.25 & 4.55 & 12.36 & 0.87 & 16.47 & 29.74 & 82.61 & 15.91 & 37.00 & 9.47 & 145\\

\bottomrule

\end{tabular}

}
\caption{\textbf{(Gemini)}}
\label{tab:different_kg_results}
\end{table*}

==> tables/gpt4_results.tex <==
\begin{table}[h]
\centering
\resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{lccccc}
    \toprule
    \textbf{} &\textbf{CON} &\textbf{INFO} & \textbf{REL} \\
    \midrule
    {\textit{\textbf{Answer}}}  & 5.45 & 5.28 & 6.88 \\
    \midrule
    \multicolumn{4}{l}{\textit{\textbf{GPT-3.5}}} \\
        ~~~\textsc{no\_kg\_no\_pres} & 4.44 & 4.34 & 6.84 \\
        ~~~\textsc{with\_kg\_no\_pres} & 4.33 & 4.23 & 6.69 \\
        ~~~\textsc{no\_kg\_with\_pres} &  5.68 & 5.91 & 6.99 \\
        ~~~\textsc{with\_kg\_with\_pres}& 5.37 & 5.80 & 5.84 \\  
        
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Evaluation results of GPT-4} with different configurations across multiple dimensions.
% The scoring system ranges from 1 to 10, focusing on Concreteness (CON), Information Richness (INFO), and Relevance and Accuracy (REL).}
(\textit{CON} for Concreteness, \textit{INFO} for Information Richness, \textit{REL} for Relevance and Accuracy).}
% The best scores are emphasized in bold, while underlined values indicate improvements over the original \textsc{answer}, showcasing the model's adaptability to different settings.}

\label{tab:results_GPT4}

\end{table}


==> tables/human_eval.tex <==
\begin{table}[hbt!]
    \centering
    \begin{center}
    \resizebox{0.475\textwidth}{!}{
    \renewcommand{\arraystretch}{1.05}
        \begin{tabular}[h]{llcccccc}
        \toprule
        \textbf{} &\textbf{CON} & \textbf{INFO} & \textbf{REL} \\
        \midrule
        % \midrule
        \multirow{1}{*}{\textit{\textbf{Answer}}}
        & 3.92 & 2.17 & 6.25\\
        \midrule
 
        \multicolumn{4}{l}{\textit{\textbf{GPT-3.5}}} \\
        ~~~\textsc{no\_kg\_no\_pres} & 3.50 & \cellcolor{yellow!25}2.25 & \cellcolor{yellow!50}6.33 \\  
        ~~~\textsc{with\_kg\_no\_pres} & 3.00 & \cellcolor{yellow!25}2.17 & 5.17 \\
        ~~~\textsc{no\_kg\_with\_pres} & \cellcolor{yellow!50}4.17 & \cellcolor{yellow!25}3.67 & 6.00 \\
        ~~~\textsc{with\_kg\_with\_pres} & \cellcolor{yellow!50}4.17 & \cellcolor{yellow!50}3.83 & 3.67 \\ 
        \midrule
        
        \multicolumn{4}{l}{\textit{\textbf{Gemini 1.0 Pro}}} \\
        ~~~\textsc{no\_kg\_no\_pres} & \cellcolor{yellow!50}5.42 & \cellcolor{yellow!25}2.33 & \cellcolor{yellow!50}\textbf{7.50} \\
        ~~~\textsc{with\_kg\_no\_pres} & 2.92 & \cellcolor{yellow!25}2.42 & 5.50 \\
        ~~~\textsc{no\_kg\_with\_pres} & \cellcolor{yellow!25}3.92 & \cellcolor{yellow!25}2.33 & 6.00 \\
        ~~~\textsc{with\_kg\_with\_pres} & \cellcolor{yellow!25}4.42 & \cellcolor{yellow!50}3.08 & 4.08 \\
        \midrule
        
        \multicolumn{4}{l}{\textit{\textbf{Llama 3}}} \\
        ~~~\textsc{no\_kg\_no\_pres} & \cellcolor{yellow!25}4.83 & \cellcolor{yellow!25}2.42 & \cellcolor{yellow!50}7.42 \\
        ~~~\textsc{with\_kg\_no\_pres} & \cellcolor{yellow!25}4.00 & \cellcolor{yellow!25}5.75 & 3.92 \\
        ~~~\textsc{no\_kg\_with\_pres} & \cellcolor{yellow!50}\textbf{5.92} & \cellcolor{yellow!25}5.25 & 4.08 \\
        ~~~\textsc{with\_kg\_with\_pres} & \cellcolor{yellow!25}4.17 & \cellcolor{yellow!50}\textbf{7.08} & 2.25 \\
        \bottomrule
        
        \end{tabular}
    }
    \end{center}
    \vspace{-0.15in}

    % \caption{\small \textbf{Human evaluation results}, where we randomly sample 30 examples. 
    % Light yellow cells denote scores that equal or exceed the baseline 'Answer' scores. 
    % Darker yellow cells highlight the highest scores within each language model. 
    % Bolded values indicate the highest scores across all configurations for each category.}

    \caption{\textbf{Human evaluation results}, where we randomly sample 30 examples. 
    Light yellow cells denote scores that equal or exceed the baseline 'Answer' scores. 
    Darker yellow cells highlight the highest scores within each language model. 
    Bolded values indicate the highest scores across all configurations for each category.}
    % The configurations tested include: 'no\_kg\_no\_pres' (without a knowledge graph and without a presentation), 'with\_kg\_no\_pres' (with a knowledge graph but without a presentation), 'no\_kg\_with\_pres' (without a knowledge graph but with a presentation), and 'with\_kg\_with\_pres' (with both a knowledge graph and a presentation). }
    % These settings explore the impact of knowledge integration and presentation data on the performance of language models in terms of concreteness, information richness, and relevance.}
    

    \label{tab:human}
    
    \vspace{-0.1in}
\end{table}

==> tables/main_results.tex <==
% \begin{table*}[hbt!]
% % \vspace{-0.1in}
% \small
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llccccccccccca}
% \toprule

% % & \multicolumn{4}{c}{\bf N-gram based} & \multicolumn{1}{c}{\bf Faithful based}  & \multicolumn{1}{c}{\bf Model based} & \multicolumn{4}{c}{\bf Terms} \\
% % \cmidrule(l{2pt}r{2pt}){2-6} \cmidrule(l{2pt}r{2pt}){7} \cmidrule(l{2pt}r{2pt}){8} \cmidrule(l{2pt}r{2pt}){9-11} \cmidrule(l{2pt}r{2pt}){11-14}
% % & \multicolumn{4}{c}{\bf N-gram based} & \multicolumn{1}{c}{\bf Faithful} \\
% % \cmidrule(l{2pt}r{2pt}){2-6} \cmidrule(l{2pt}r{2pt}){1}

% & \multicolumn{2}{c}{} & \multicolumn{5}{c}{\bf ROUGE} & \multicolumn{2}{c}{\bf} & \multicolumn{3}{c}{\bf Term} \\
% \cmidrule(l{2pt}r{2pt}){4-8}  \cmidrule(l{2pt}r{2pt}){11-13}

% % kg, speech
% \textbf{} & \textbf{KG} & \textbf{Presentation} & \textbf{Rough1} & \textbf{Rough2} & \textbf{RoughL} & \textbf{BLEU} & \textbf{METEOR} & \textbf{QuestEval} & \textbf{BERTscore} & \textbf{OTR} & \textbf{TQA} & \textbf{TANQ} & \textbf{Length} \\

% \midrule
% \midrule

% \multirow{3}{*}{\textit{\textbf{Gemini}}}  
% & x & x & 29.79 & 5.00 & 15.10 & 0.83 & 18.28 & 32.57 & 83.63 & 17.72 & 35.99 & 10.37 & 161\\
% % & $\vee$(part) & x & 27.35 & 4.59 & 14.03 & 0.60 & 18.34 & 31.89 & 83.67 \\
% % & \multirow{5}{*}{[with constraint]} & $\vee$(part) & x & 31.85 & 5.20 & 15.43 & 0.79 & 17.83 & 32.51 & 83.53 \\
% % & & $\vee$(kg1) & x & 22.69 & 3.57 & 12.31 & 0.47 & 17.11 & 29.56 & 83.04 \\
% % & & $\vee$(kg2) & x & 25.50 & 4.23 & 13.64 & 0.73 & 18.16 & 30.97 & 83.54 \\
% % & & $\vee$(kg3) & x & 24.88 & 3.95 & 13.27 & 0.51 & 18.19 & 30.92 & 83.53 \\ &
% & $\vee$ & x & 27.26 & 4.96 & 14.43 & 0.81 & 18.86 & 31.65 & 83.86 & 15.61 & 41.7 & 6.47 & 107\\
% & x & $\vee$ & 24.49 & 4.57 & 12.63 & &  & & 83.01 & 15.47 & 36.61 & 7.32 & 103\\
% & $\vee$ & $\vee$ & 24.25 & 4.55 & 12.36 & 0.87 & 16.47 & 29.74 & 82.61 & 15.91 & 37.0 & 9.47 & 145\\
% % & $\vee$(kg1) & $\vee$ & 15.50 & 2.22 & 9.19 & 0.27 & 13.33 & 25.42 & 81.57 \\
% % & $\vee$(kg2) & $\vee$ & 22.28 & 3.84 & 12.02 & 0.44 & 16.94 & 28.33 & 82.55 \\
% % & $\vee$(kg3) & $\vee$ & 21.01 & 3.69 & 11.53 & 0.56 & 16.71 & 28.20 & 82.67 \\

% \midrule

% \multirow{3}{*}{\textit{\textbf{Gpt3.5}}}  
% & x & x & 28.73 & 4.65 & 14.73 & 0.73 & 19.29 & 32.18 & 83.79 \\
% & $\vee$ & x & 27.11 & 4.35 & 14.12 & 0.54 & 19.33 & 31.77 & 83.70 \\
% & x & $\vee$ & \textbf{29.98} & \textbf{5.12} & 14.89 & \textbf{0.88} & 17.54 & 32.09 & 83.46 \\
% & $\vee$ & $\vee$ & 27.85 & 4.28 & 13.86 & 0.73 & 16.66 & 30.18 & 82.97 \\

% \midrule

% \multirow{4}{*}{\textit{\textbf{Llama3 \scriptsize(8B)}}}  
% & x & x & \textbf{34.68} & \textbf{6.55} & \textbf{15.60} & \textbf{1.41} & 19.89 & \textbf{33.81} & \textbf{84.10} \\
% & $\vee$ & x & 28.95 & 4.72 & 13.55 & 0.82 & 14.69 & 28.55 & 82.27 \\
% & x & $\vee$ & 25.67 & 3.68 & 12.04 & 0.52 & 13.38 & 26.06 & 81.54 \\
% & $\vee$ & $\vee$ & 28.28 & 4.18 & 13.30 & 0.54 & 13.77 & 29.57 & 81.81 \\

% \bottomrule

% \end{tabular}

% }
% \caption{\textbf{Main results of language model prompting with kg and speech constraints}. Best scores are emphasized in bold.}
% \label{tab:main_results}
% \end{table*}

\begin{table*}[t!]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccca}
% \begin{tabular}{l|cc|ccccccc|ccca}
\toprule

& \multicolumn{2}{c}{} & \multicolumn{4}{c}{\bf N-gram Based} & \multicolumn{3}{c}{\bf Contextual Semantics} & \multicolumn{3}{c}{\bf Term} \\
\cmidrule(l{2pt}r{2pt}){4-7} \cmidrule(l{2pt}r{2pt}){8-10}  \cmidrule(l{2pt}r{2pt}){11-13}

\textbf{} & \textbf{KG} & \textbf{PRE} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{BLEU} & \textbf{METEOR} & \textbf{QuestEval} & \textbf{BERTscore} & \textbf{CDR} & \textbf{QDR} & \textbf{IIR} & \textbf{Length} \\

\midrule
% \midrule
\multirow{4}{*}{\textit{\textbf{Gemini}}}  
& \xmark &  \xmark & 29.79 & 5.00 & 15.10 & 0.83 & 18.28 & 32.57 & 83.63 & 17.72 & 35.99 & 10.37 & 161\\
\noalign{\vskip 0.5ex}\cdashline{2-14}\noalign{\vskip 0.75ex} % dotted line
& \cmark &  \xmark & 27.26 & 4.96 & 14.43 & 0.81 & \cellcolor{green!25}18.86 & 31.65 & \cellcolor{green!25}83.86 & 15.61 & \cellcolor{green!25}41.70 & 6.47 & 107\\
&  \xmark & \cmark & 24.49 & 4.57 & 12.63 & 0.84 & 17.52 & 28.68 & 83.01 & 15.47 & \cellcolor{green!25}36.61 & 7.32 & 103\\
& \cmark & \cmark & 24.25 & 4.55 & 12.36 & \cellcolor{green!25}0.87 & 16.47 & 29.74 & 82.61 & 15.91 & \cellcolor{green!25}37.00 & 9.47 & 145\\
\midrule


\multirow{4}{*}{\textit{\textbf{GPT-3.5}}}
& \xmark & \xmark & 28.73 & 4.65 & 14.73 & 0.73 & 19.29 & 32.18 & 83.79 & 17.11 & 40.79 & 8.58 & 128 \\
\noalign{\vskip 0.5ex}\cdashline{2-14}\noalign{\vskip 0.75ex} % dotted line
& \cmark & \xmark & 27.11 & 4.35 & 14.12 & 0.54 & \cellcolor{green!25}19.33 & 31.77 & 83.70 & \cellcolor{green!25}17.69 & 41.79 & \cellcolor{green!25}8.72 & 112 \\
& \xmark & \cmark & \cellcolor{green!25}29.98 & \cellcolor{green!25}5.12 & \cellcolor{green!25}14.89 & \cellcolor{green!25}0.88 & 17.54 & 32.09 & 83.46 & \cellcolor{green!25}22.35 & 45.41 & \cellcolor{green!25}14.60 & 186\\
& \cmark & \cmark & 27.85 & 4.28 & 13.86 & 0.73 & 16.66 & 30.18 & 82.97 & \cellcolor{green!25}24.06 & 38.69 & \cellcolor{green!25}18.54 & 185\\

\midrule

\multirow{4}{*}{\textit{\textbf{Llama3 \scriptsize(8B)}}}
& \xmark & \xmark & 34.68 & 6.55 & 15.60 & 1.41 & 19.89 & 33.81 & 84.10 & 19.13 & 43.62 & 9.77 & 174\\
\noalign{\vskip 0.5ex}\cdashline{2-14}\noalign{\vskip 0.75ex} % dotted line
& \cmark &  \xmark & 28.95 & 4.72 & 13.55 & 0.82 & 14.69 & 28.55 & 82.27 & 16.53 & 24.21 & \cellcolor{green!25}13.65 & 313\\
& \xmark & \cmark & 25.67 & 3.68 & 12.04 & 0.52 & 13.38 & 26.06 & 81.54 & 19.53 & 21.41 & \cellcolor{green!25}17.62 & 271 \\
& \cmark & \cmark & 28.28 & 4.18 & 13.30 & 0.54 & 13.77 & 29.57 & 81.81 & 19.08 & 18.62 &\cellcolor{green!25} 17.31 & 303\\


\bottomrule

\end{tabular}

}
\caption{\textbf{Main results of language model prompting with kg and speech constraints}. PRE denotes Presentation. Light green indicates scores that exceed the baseline (no knowledge graph, no presentation)}
% , while dark green marks the highest scores within each model.}
\label{tab:main_results}
\end{table*}


